ShortCoder: Knowledge-Augmented Syntax Optimization for Token-Efficient Code Generation

Code generation tasks aim to automate the conversion of user requirements into executable code, significantly reducing manual development efforts and enhancing software productivity. The emergence of large language models (LLMs) has significantly advanced code generation, though their efficiency is still impacted by certain inherent architectural constraints. Each token generation necessitates a complete inference pass, requiring persistent retention of contextual information in memory and escalating resource consumption. While existing research prioritizes inference-phase optimizations such as prompt compression and model quantization, the generation phase remains underexplored. To tackle these challenges, we propose a knowledge-infused framework named ShortCoder, which optimizes code generation efficiency while preserving semantic equivalence and readability. In particular, we introduce: (1) ten syntax-level simplification rules for Python, derived from AST-preserving transformations, achieving 18.1% token reduction without functional compromise; (2) a hybrid data synthesis pipeline integrating rule-based rewriting with LLM-guided refinement, producing ShorterCodeBench, a corpus of validated tuples of original code and simplified code with semantic consistency; (3) a fine-tuning strategy that injects conciseness awareness into the base LLMs. Extensive experimental results demonstrate that ShortCoder consistently outperforms state-of-the-art methods on HumanEval, achieving an improvement of 18.1%-37.8% in generation efficiency over previous methods while ensuring the performance of code generation.

==> fig_rules.tex <==
% Required packages

% Figure 1: Multiple Variable Assignment Simplification


% Figure 2: Operator Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
x = x + 1
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
x += 1
\end{lstlisting}
\end{minipage}
\caption{Simplification using compound assignment operator.}
\label{fig:rule2}
\end{figure}

% Figure 3: Conditional Statement Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
if condition:
    flag = True
else:
    flag = False
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
flag = condition
\end{lstlisting}
\end{minipage}
\caption{Simplification of conditional assignment.}
\label{fig:rule3}
\end{figure}

% Figure 4: Multiple Condition Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
if condition1:
    result = 'A'
else:
    if condition2:
        result = 'B'
    else:
        result = 'C'
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
if condition1:
    result = 'A'
elif condition2:
    result = 'B'
else:
    result = 'C'
\end{lstlisting}
\end{minipage}
\caption{Simplification of nested conditionals using \texttt{elif}.}
\label{fig:rule4}
\end{figure}

% Figure 5: For Loop Simplification (List Comprehension)
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
result = []
for x in data:
    result.append(x * 2)
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
result = [x * 2 for x in data]
\end{lstlisting}
\end{minipage}
\caption{For loop simplification using list comprehension.}
\label{fig:rule5}
\end{figure}

% Figure 6: Multiple Delete Statements Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
del a
del b
del c
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
del a, b, c
\end{lstlisting}
\end{minipage}
\caption{Combining multiple delete statements.}
\label{fig:rule6}
\end{figure}

% Figure 7: String Formatting Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
msg = "Hello " + name + "!"
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
msg = "Hello {}!".format(name)
\end{lstlisting}
\end{minipage}
\caption{String concatenation simplified with \texttt{str.format()}.}
\label{fig:rule7}
\end{figure}

% Figure 8: Dictionary Mapping Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
if key in dictionary:
    value = dictionary[key]
else:
    value = default
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
value = dictionary.get(key, default)
\end{lstlisting}
\end{minipage}
\caption{Simplification using dictionary \texttt{get()} method.}
\label{fig:rule8}
\end{figure}

% Figure 9: File Reading Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
f = open('file.txt', 'r')
data = f.read()
f.close()
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
with open('file.txt', 'r') as f:
    data = f.read()
\end{lstlisting}
\end{minipage}
\caption{File reading simplified with \texttt{with open()}.}
\label{fig:rule9}
\end{figure}

% Figure 10: File Writing Simplification
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Original Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
f = open('file.txt', 'w')
f.write("Hello")
f.close()
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
\centering
\textbf{Simplified Code}
\begin{lstlisting}[language=Python, basicstyle=\ttfamily\small]
with open('file.txt', 'w') as f:
    f.write("Hello")
\end{lstlisting}
\end{minipage}
\caption{File writing simplified with \texttt{with open()}.}
\label{fig:rule10}
\end{figure}

